A One-Layer Decoder-Only Transformer is a Two-Layer RNN: With an Application to Certified Robustness

This paper reveals a key insight that a one-layer decoder-only Transformer is equivalent to a two-layer Recurrent Neural Network (RNN). Building on this insight, we propose ARC-Tran, a novel approach for verifying the robustness of decoder-only Transformers against arbitrary perturbation spaces. Compared to ARC-Tran, current robustness verification techniques are limited either to specific and length-preserving perturbations like word substitutions or to recursive models like LSTMs. ARC-Tran addresses these limitations by meticulously managing position encoding to prevent mismatches and by utilizing our key insight to achieve precise and scalable verification. Our evaluation shows that ARC-Tran (1) trains models more robust to arbitrary perturbation spaces than those produced by existing techniques and (2) shows high certification accuracy of the resulting models.

==> tables/ablation.tex <==
\begin{table}[t]
\centering
    \caption{Ablation results focusing on \emph{context-free perturbations}.}
    \vspace{-0.5em}
\resizebox{0.8\columnwidth}{!}{
\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1} 
\begin{tabular}{l rrr}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{Overall Average} \\ 
\cmidrule(lr){2-4} 
& \npsk & \rpsk & \rdrop  \\
\midrule
$[0]:\lossclm$ & 23.67 & 7.52 & 68.23\\
% $\lossdataaug$ & 18.28 & 7.93 & 18.28 & 7.41 & 30.56 & 9.35 & 30.56 & 19.12 & 24.42 & 10.95 & 44.84 \\
$[1]:\lossdataaug$ & 24.10 & 10.64 & 55.85 \\
$[2]:\lossmdataaug$ & 23.77 & 11.10 & 53.30\\
$[3]:\lossmdataaug (p=20\%)$  & 24.60 & 10.48 & 57.40\\
$[4]:\lossmbatchaug$ & 24.90 & 11.01 & 55.78\\
\rowcolor{gray!30}$[5]:\lossmbatchaug + \lossalp$ &  24.67 & 11.48 & 53.47 \\
$[6]:\lossclm + \losscontraseq$ & 23.80 & 7.79 & 67.27 \\
$[7]:[5] + \losscontratoken$ & 23.52 & 11.18 & 52.47 \\
$[8]:[5] + \losscontraseq$ & 24.64 & 11.51 & 53.29 \\
\bottomrule
\end{tabular}
}
\vspace{-1em}
    \label{tab:ablation_results_free}
\end{table}


\begin{table}[t]
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.2}
\centering
    \caption{Ablation results focusing on \emph{context-sensitive} perturbations.}
   \vspace{-0.5em}
\resizebox{0.8\columnwidth}{!}{
\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1} 
\begin{tabular}{l rrr}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{Overall Average} \\ 
\cmidrule(lr){2-4} 
& \npsk & \rpsk & \rdrop  \\
\midrule
$[0]:\lossclm$ & 23.67 & 7.52 & 68.23\\
$[1]:\lossmbatchaug$ & 24.83 & 10.75 & 56.71\\
\rowcolor{gray!30}$[2]:\lossmbatchaug + \lossalpdrop$ & 24.82 & 10.94 & 55.92 \\
$[3]:\lossmbatchaug + \losscontraname$ & 24.60 & 10.87 & 55.81\\
$[4]:[2] + \losscontraname$ & 24.66 & 10.80 & 56.20 \\
$[5]:[4] + \losscontratoken$ & 24.42 & 10.42 & 57.33 \\
\bottomrule
\end{tabular}
}
 \vspace{-1em}
    \label{tab:ablation_results_sensitive}
\end{table}


==> tables/ablation_full.tex <==
\begin{table*}
\setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.2}
\centering
 \caption{Ablation results of CodeGen-350M focusing on \emph{context-free perturbations}, i.e., we apply $\lossdataaug$ loss to the context-sensitive perturbations except for the baseline $\lossclm$.}
 \vspace{-0.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l rr rr rr rr rrr}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Docstring} & 
\multicolumn{2}{c}{Function} & \multicolumn{2}{c}{Syntax} & \multicolumn{2}{c}{Format} & \multicolumn{3}{c}{Overall Average} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  \cmidrule(lr){10-12} 
& \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \rdrop  \\
\midrule
$[0]\lossclm$ & 18.10 & 6.19 & 18.10 & 6.47 & 29.24 & 1.46 & 29.24 & 15.96 & 23.67 & 7.52 & 68.23\\
% $\lossdataaug$ & 18.28 & 7.93 & 18.28 & 7.41 & 30.56 & 9.35 & 30.56 & 19.12 & 24.42 & 10.95 & 44.84 \\
$[1]\lossdataaug$ & 18.10 & 7.45 & 18.10 & 7.94 & 30.11 & 8.59 & 30.11 & 18.58 & 24.10 & 10.64 & 55.85 \\
$[2]\lossmdataaug$ & 17.57 & 8.12 & 17.57 & 7.91 & 29.96 & 9.31 & 29.96 & 19.07 & 23.77 & 11.10 & 53.30\\
$[3]\lossmdataaug (p=0.2)$ & 17.91 & 7.36 & 17.91 & 7.84 & 31.30 & 8.88 & 31.30 & 17.86 & 24.60 & 10.48 & 57.40\\
$[4]\lossmbatchaug$ & 18.24 & 7.17 & 18.24 & 8.21 & 31.56 & 10.02 & 31.56 & 18.65 & 24.90 & 11.01 & 55.78\\
\rowcolor{gray!30}$[5]\lossmbatchaug + \lossalp$ & 18.03 & 7.38 & 18.03 & 8.19 & 31.30 & 11.92 & 31.30 & 18.44 & 24.67 & 11.48 & 53.47\\
$[6]\lossclm + \losscontraseq$ & 17.52 & 7.17 & 17.52 & 7.56 & 30.07 & 1.37 & 30.07 & 15.06 & 23.80 & 7.79 & 62.27 \\
$[7]\lossmbatchaug + \lossalp + \losscontratoken$ & 17.33 & 7.12 & 17.33 & 8.03 & 29.72 & 11.46 & 29.72 & 18.10 & 23.52 & 11.18 & 52.47 \\
$[8]\lossmbatchaug + \lossalp + \losscontraseq$ & 17.98 & 7.38 & 17.98 & 8.15 & 31.30 & 11.81 & 31.30 & 18.70 & 24.64 & 11.51 & 53.29 \\
$[9]\lossmbatchaug + \lossalp(\emph{On}+\emph{Co}) + \losscontratoken + \losscontraseq$ & 17.36 & 7.35 & 17.36 & 7.91 & 29.42 & 11.12 & 29.42 & 18.09 & 23.39 & 11.12 & 52.46\\
$[10]\lossmbatchaug + \lossalp(\emph{On}+\emph{Al}) + \losscontratoken + \losscontraseq$ & 17.31 & 7.33 & 17.31 & 7.80 & 29.77 & 11.48 & 29.77 & 18.12 & 23.54 & 11.18 & 52.51 \\
$[11]\lossmbatchaug + \lossalp(\emph{Bo}+\emph{Co}) + \losscontratoken + \losscontraseq$ & 16.87 & 7.19 & 16.87 & 7.72 & 29.40 & 11.07 & 29.40 & 17.82 & 23.14 & 10.95 & 52.68 \\
$[12]\lossmbatchaug + \lossalp(\emph{Bo}+\emph{Al}) + \losscontratoken + \losscontraseq$ & 16.70 & 7.15 & 16.70 & 7.77 & 29.54 & 11.41 & 29.54 & 17.62 & 23.12 & 10.99 & 52.47 \\
\bottomrule
\end{tabular}
}
   \vspace{-1em}
    \label{tab:ablation_results_free_full}
\end{table*}


\begin{table*}
\setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.2}
\centering
 \caption{Ablation results of CodeGen-350M focusing on \emph{context-sensitive} perturbations, i.e., we apply $\lossdataaug$ loss to the context-free perturbations except for the baseline $\lossclm$.}
 \vspace{-0.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l rr rr rr rr rrr}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Docstring} & 
\multicolumn{2}{c}{Function} & \multicolumn{2}{c}{Syntax} & \multicolumn{2}{c}{Format} & \multicolumn{3}{c}{Overall Average} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  \cmidrule(lr){10-12} 
& \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \rperct  \\
\midrule
$[0]\lossclm$ & 18.10 & 6.19 & 18.10 & 6.47 & 29.24 & 1.46 & 29.24 & 15.96 & 23.67 & 7.52 & 31.77\\
$[1]\lossmbatchaug$ & 18.68 & 8.19 & 18.68 & 8.56 & 30.98 & 7.72 & 30.98 & 18.54 & 24.83 & 10.75 & 43.29\\
\rowcolor{gray!30}$[2]\lossmbatchaug + \lossalpdrop$ & 18.80 & 8.44 & 18.80 & 8.37 & 30.84 & 8.00 & 30.84 & 18.98 & 24.82 & 10.94 & 44.08 \\
$[3]\lossmbatchaug + \losscontraname$ & 18.65 & 8.14 & 18.65 & 8.49 & 30.54 & 7.94 & 30.54 & 18.91 & 24.60 & 10.87 & 44.19\\
$[4]\lossmbatchaug + \lossalpdrop + \losscontraname$ & 18.63 & 8.12 & 18.63 & 8.26 & 30.69 & 7.82 & 30.69 & 18.98 & 24.66 & 10.80 & 43.80 \\
$[5]\lossmbatchaug + \lossalpdrop + \losscontraname + \losscontratoken$ & 18.31 & 7.79 & 18.31 & 7.80 & 30.53 & 8.17 & 30.53 & 17.93 & 24.42 & 10.42 & 42.67 \\
$[6]\lossmbatchaug + \lossalpdrop (\emph{All})$ & 18.07 & 8.66 & 18.07 & 8.12 & 30.33 & 7.56 & 30.33 & 18.88 & 24.20 & 10.80 & 44.63 \\
$[7]\lossmbatchaug + \lossalpdrop (\emph{AllS})$ & 18.37 & 8.12 & 18.37 & 8.73 & 30.51 & 7.49 & 30.51 & 18.08 & 24.44 & 10.61 & 43.42 \\
\bottomrule
\end{tabular}
}
\vspace{-1em}
    \label{tab:ablation_results_sensitive_full}
\end{table*}


==> tables/equations.tex <==
\begin{table*}
    \centering
    \begin{tabular}{l}
         \toprule
         Equations\\
         \midrule
$
\begin{aligned}
   \lossmbatchaug = \sum_{1\le i \le b, a \in \bernoulli{p}} a(\lossclm(\bfx_i) + \lossclm(\pt{\bfx_i}, \pt{\mask_i})) + (1-a)\lossclm(\bfx_i)
\end{aligned}
$
\\
          \\
         \bottomrule
    \end{tabular}
    \caption{Definitions of the robust training losses.}
    \label{tab:my_label}
\end{table*}

==> tables/extended_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.2}
\centering
\vspace{0.1em}
    \caption{Robustness evaluation for each category of perturbations on combined HumanEval and MBPP datasets. We highlight in gray the top four perturbation types that we have achieved the most improvements over the baseline $\lossclm$.}
    % \vspace{-0.5em}
\resizebox{0.9\linewidth}{!}{

    \begin{tabular}{l|l|rrr|rrr|rrr}
    \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{Categories}} & \multicolumn{1}{c|}{\multirow{2}{*}{Transformations}} & \multicolumn{3}{c|}{CodeGen 350M}                                                               & \multicolumn{3}{c|}{CodeGen 2B}                                                                 & \multicolumn{3}{c}{CodeGen 6B}                                                                 \\ \cline{3-11} 
        \multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{l}{$\lossclm$} & \multicolumn{1}{l}{$\lossdataaug$} & \multicolumn{1}{l|}{Ours} & \multicolumn{1}{l}{$\lossclm$} & \multicolumn{1}{l}{$\lossdataaug$} & \multicolumn{1}{l|}{Ours} & \multicolumn{1}{l}{$\lossclm$} & \multicolumn{1}{l}{$\lossdataaug$} & \multicolumn{1}{l}{Ours} \\ \hline
    \multirow{2}{*}{Nominal}     
    & Regular                         & 18.10    & 18.10   & 18.33    & 32.99    & 31.62   & 31.56    & 40.07 & 37.61 & 37.91    \\
    & Partial                         & 29.24    & 30.11   & 31.04    & 46.22    & 45.96   & 45.04    & 54.46 & 52.99 & 53.16    \\ \hline
    \multirow{6}{*}{Docstring}   
    & BackTranslation                 & 17.35    & 17.66   & 17.79    & 31.6     & 29.86   & 30.53    & 38.91 & 36.75 & 37.45    \\
                                 & EnglishInflectionalVariation    & 10.98    & 10.98   & 12.50    & 23.95    & 22.93   & 23.99    & 28.35 & 27.21 & 29.02   \\
                                  & SynonymSubstitution\cellcolor{gray!30}              & 7.03\cellcolor{gray!30}      & 8.98\cellcolor{gray!30}     & 11.20\cellcolor{gray!30}     & 17.35\cellcolor{gray!30}     & 18.95\cellcolor{gray!30}    & 21.18\cellcolor{gray!30}     & 22.11\cellcolor{gray!30}     & 22.78\cellcolor{gray!30}    & 25.06\cellcolor{gray!30}     \\
                                 & TenseTransformationFuture       & 17.49    & 17.72   & 18.33    & 32.07    & 31.34   & 31.35    & 39.79 & 37.38 & 37.63    \\
                                 & TenseTransformationPast         & 18.12    & 18.51   & 18.63    & 32.55    & 31.21   & 31.55    & 39.40 & 37.28 & 37.70   \\
                                 & WorstCase                       & 6.19     & 7.45    & 9.72     & 15.78    & 17.07   & 19.21    & 20.21 & 20.51 & 23.13    \\ \hline
    \multirow{7}{*}{Function}    & RenameButterFinger          & 11.56    & 11.79   & 11.90    & 23.88    & 23.15   & 23.34    & 29.86 & 28.95 & 28.82    \\
                                 & RenameCamelCase             & 17.70    & 17.72   & 18.15    & 34.08    & 32.06   & 32.37    & 40.47 & 37.91 & 38.59    \\
                                 & RenameChangeChar \cellcolor{gray!30}             & 8.54\cellcolor{gray!30}      & 10.39\cellcolor{gray!30}    & 10.33\cellcolor{gray!30}     & 20.14\cellcolor{gray!30}     & 20.91\cellcolor{gray!30}    & 20.88\cellcolor{gray!30}     & 27.03\cellcolor{gray!30}     & 26.63\cellcolor{gray!30}    & 26.84\cellcolor{gray!30}     \\
                                 & RenameInflectionalVariation & 14.11    & 14.76   & 15.20    & 28.56    & 27.87   & 28.19    & 33.36 & 32.48 & 33.66    \\
                                 & RenameSwapChar              & 11.92    & 11.86   & 12.20    & 24.69    & 24.17   & 24.25    & 31.44 & 29.81 & 29.49    \\
                                 & RenameSynonymSub            & 12.07    & 12.95   & 13.04    & 24.97    & 24.50   & 24.82    & 30.14 & 29.95 & 30.47    \\
                                 & WorstCase                       & 6.47     & 7.94    & 8.05     & 16.41    & 16.61   & 17.12    & 22.18 & 21.88 & 22.53    \\ \hline
    \multirow{8}{*}{Syntax}      & DeadCodeInsertion                & 1.92     & 15.83   & 20.77    & 3.87     & 33.25   & 32.93    & 3.32 & 38.86 & 41.16    \\
                                 &  DeadCodeInsertionLast \cellcolor{gray!30}             & \cellcolor{gray!30} 9.24     & \cellcolor{gray!30} 31.55   & \cellcolor{gray!30} 32.69    & \cellcolor{gray!30} 13.90    & \cellcolor{gray!30} 48.26   & \cellcolor{gray!30} 49.47    & \cellcolor{gray!30} 14.39    & \cellcolor{gray!30} 55.13    & \cellcolor{gray!30} 55.15    \\
                                 & ForWhileTransformer             & 27.08    & 26.99   & 29.16    & 43.78    & 42.76   & 41.90    & 50.35 & 50.49 & 50.81    \\
                                 & OperandSwap                     & 27.80    & 26.91   & 29.12    & 44.50    & 43.32   & 43.15    & 51.53 & 51.46 & 51.60    \\
                                 & VarRenamerCB                    & 26.52    & 25.85   & 27.72    & 44.60    & 42.85   & 42.04    & 49.12 & 48.17 & 49.35    \\
                                 & VarRenamerNaive                 & 24.99    & 26.31   & 26.22    & 42.53    & 41.20   & 41.09    & 49.28 & 49.05 & 48.14    \\
                                 & VarRenamerRN                    & 14.75    & 15.41   & 15.78    & 31.65    & 31.48   & 30.56    & 37.07 & 37.07 & 36.03    \\
                                 & WorstCase                       & 1.46     & 8.59    & 10.67    & 2.43     & 22.86   & 21.92    & 2.58 & 27.66 & 27.70    \\ \hline
    \multirow{4}{*}{Format}      & Doc2Comments                    & 25.48    & 27.66   & 28.75    & 45.36    & 44.29   & 42.67    & 50.28 & 51.27 & 51.30    \\
                                 & NewLineInsertion \cellcolor{gray!30}                              & \cellcolor{gray!30} 20.44    & \cellcolor{gray!30} 22.32   & \cellcolor{gray!30} 25.54    & \cellcolor{gray!30} 35.52    & \cellcolor{gray!30} 37.86   & \cellcolor{gray!30} 37.91    & \cellcolor{gray!30} 39.74    & \cellcolor{gray!30} 46.19   & \cellcolor{gray!30} 48.58    \\
                                 & SplitLine                           & 27.07    & 28.42   & 30.04    & 44.60    & 45.18   & 43.44    & 52.07 & 52.16 & 51.83    \\
                                 & WorstCase                       & 15.96    & 18.58   & 21.58    & 32.00    & 34.50   & 34.36    & 35.80 & 42.18 & 44.87    \\ \bottomrule

    \end{tabular}





}
% \vspace{-1em}
    \label{tab:overall_granular_results}
\end{table*}



==> tables/main_results.tex <==
% % \usepackage{tabularray}
% \begin{table*}
% % \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.2}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ll|rrr|rrrr|rrrr}
% \toprule
% \multicolumn{2}{c|}{\multirow{2}{*}{Model \& Methods}}  &  \multicolumn{3}{c|}{StarCoder} & 
% % \multicolumn{3}{c|}{CodeGen-6B} & 
% \multicolumn{4}{c|}{CodeGen-2B} & \multicolumn{4}{c}{CodeGen-350M} \\ 
% & & Ori & $\lossdataaug$ & Ours 
% % & $\lossclm$ & $\lossdataaug$ & Ours 
% & Ori & $\lossclm$ & $\lossdataaug$ & Ours & Ori & $\lossclm$ & $\lossdataaug$ & Ours\\

% \midrule
% \multirow{3}{*}{Docstring} & \npsk & 
% 42.34 & 43.95 & 43.69 & % starcoder
% 31.27 & \textbf{32.99} & 31.62 & 31.56 & %codegen2B
% 17.10 & 18.10 & 18.10 & \textbf{18.33}\\ %codegen350M
% % 17.10 & 18.10 & 18.28 & \textbf{18.33}\\ %codegen350M
% & \rpsk & 
% 17.61 & 26.66 & 23.85 &
% 11.04 & 15.78 & 17.62 & \textbf{19.21} &
% 3.57 & 6.19 & 7.45 & \textbf{9.72}\\
% % 3.57 & 6.19 & 7.93 & \textbf{9.72}\\
% & \rperct & 
% 41.59 & 60.66 & & 
% 35.31 & 47.83 & 55.72 & \textbf{60.87} & 
% 20.88 & 34.17 & 41.16 & \textbf{53.03} \\
% % 20.88 & 34.17 & 43.38 & \textbf{53.03} \\
% \hline

% \multirow{3}{*}{Function} & \npsk & 
% 42.34 & 43.95 & 43.69 & 
% 31.27 & \textbf{32.99} & 31.62 & 31.56 & 
% 17.10 & 18.10 & 18.10 & \textbf{18.33}\\
% % 17.10 & 18.10 & 18.28 & \textbf{18.33}\\
% & \rpsk & 
% 17.50 & 27.75 & 24.36 &
% 9.75 & 16.41 & 16.61 & \textbf{17.12} & 
% 3.06 & 6.47 & 7.94 & \textbf{8.05}\\
% % 3.06 & 6.47 & 7.41 & \textbf{8.05}\\
% & \rperct & 
% 41.34 & 63.14 & & 
% 31.18 & 49.74 & 52.53 & \textbf{54.25} & 
% 17.89 & 35.73 & 43.86 & \textbf{43.92}\\
% % 17.89 & 35.73 & 40.54 & \textbf{43.92}\\
% \hline

% \multirow{3}{*}{Syntax} & \npsk & 
% 59.74 & 58.58 & 58.65 & 
% 44.82 & \textbf{46.22} & 45.96 & 45.04 & 
% 26.75 & 29.24 & 30.11 & \textbf{31.04}\\
% % 26.75 & 29.24 & 30.56 & \textbf{31.04}\\
% & \rpsk & 
% 2.48 & 32.21 & 22.22 &
% 1.63 & 2.43 & \textbf{22.86} & 21.92 & 
% 1.11 & 1.46 & 8.59 & \textbf{10.67} \\
% % 1.11 & 1.46 & 9.35 & \textbf{10.67} \\
% & \rperct & 4.15 & 66.30 & &
% 3.64 & 5.26 & \textbf{49.74} & 48.67 & 
% 4.15 & 4.99 & 28.53 & \textbf{34.38} \\
% % 4.15 & 4.99 & 30.60 & \textbf{34.38} \\
% \hline

% \multirow{3}{*}{Format} & \npsk & 
% 59.74 & 58.58 & 58.65 &
% 44.82 & \textbf{46.22} & 45.96 & 45.04 & 
% 26.75 & 29.24 & 30.11 & \textbf{31.04}\\
% % 26.75 & 29.24 & 30.56 & \textbf{31.04}\\
% & \rpsk & 35.59 & 37.79 & 38.00 &
% 24.45 & 32.00 & \textbf{34.50} & 34.36 &
% 9.54 & 15.96 & 18.58 & \textbf{21.58}\\
% % 9.54 & 15.96 & 19.12 & \textbf{21.58}\\
% & \rperct & 59.58 & 64.51 & &
% 54.55 & 69.23 & 75.07 & \textbf{76.29} & 
% 35.66 & 54.57 & 61.71 & \textbf{69.52}\\
% % 35.66 & 54.57 & 62.67 & \textbf{69.52}\\

 
% \bottomrule
% \end{tabular}
% }
%     \caption{Main Results. Robust evaluation of StarCoder, CodeGen-2B, and CodeGen-350M on a union of HumanEval and MBPP datasets. Our approach uses the setting $\lossmbatchaug + \lossalp + \lossalpdrop$.}
%     \label{tab:main_results}
% \end{table*}


\begin{table*}
\centering
    \caption{Robust evaluation of CodeGen-6B, CodeGen-2B, and CodeGen-350M on a union of HumanEval and MBPP datasets. Our best approach uses the setting $\lossmbatchaug + \lossalp + \lossalpdrop$. We show the statistical significance between our approach and $\lossdataaug$ using the paired-t test with $^*$ denoting $p<0.05$ and $^{**}$ denoting $p<0.01$. \npsk and \rpsk are higher the better. \rdrop is lower the better.}
    \vspace{-0.5em}
\resizebox{0.8\linewidth}{!}{
\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1} 
\begin{tabular}{ll rr rr rr rr rrr}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Model \& Methods}}  & \multicolumn{2}{c}{Docstring} & 
\multicolumn{2}{c}{Function} & \multicolumn{2}{c}{Syntax} & \multicolumn{2}{c}{Format} & \multicolumn{3}{c}{Overall Average} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}  \cmidrule(lr){11-13} 
& & \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \npsk & \rpsk & \rdrop  \\

\midrule

% \multirow{3}{*}{StarCoder} 
% & Ori($\lossclm$) & 42.34 & 17.61 & 42.34 & 17.50 & 59.74 & 2.48 & 59.74 & 35.59 & 51.04 & 18.30 & 35.85\\
% & $\lossdataaug$ & 43.95 & 26.66 & 43.95 & 27.75 & 58.58 & 32.21 & 58.58 & 37.79 & 51.27 & 31.10 & 60.66\\
% & \cellcolor{gray!30} Ours &  \\
% \midrule

\multirow{4}{*}{CodeGen-6B}
& Ori & 35.96 & 12.83 & 35.96 & 14.36 & 52.72 & 2.20 & 52.72 & 25.47 & 44.34 & 13.71 & 69.08\\
& $\lossclm$ & 40.07 & 20.21 & 40.07 & 22.18 & 54.91 & 2.58 & 54.91 & 35.80 & \textbf{47.27} &  20.19 & 57.29\\
& $\lossdataaug$ & 37.61 & 20.51 & 37.61 & 21.88 & 52.99 & 27.66 &  52.99 & 42.18 & 45.30 & 28.06 & 38.06\\
& \cellcolor{gray!30} Ours & \cellcolor{gray!30} 37.91 & \cellcolor{gray!30} \textbf{$^{**}$23.13} & \cellcolor{gray!30} 37.91 & \cellcolor{gray!30} \textbf{22.53} & \cellcolor{gray!30} 53.16 & \cellcolor{gray!30} \textbf{27.70} & \cellcolor{gray!30} 53.16 & \cellcolor{gray!30} \textbf{$^{**}$44.87} & \cellcolor{gray!30} 45.54 & \cellcolor{gray!30} \textbf{29.56} & \cellcolor{gray!30} \textbf{35.09} \\
% & $\lossclm$ & 39.68 & 19.47 & 39.68 & \textbf{22.20} & 54.48 & 2.64 & 54.48 & 35.89 & \textbf{47.08} &  20.05 & 57.41\\
% & $\lossdataaug$ & 36.91 & 20.62 & 36.91 & 21.62 & 53.20 & 27.35 &  53.20 & \textbf{42.25} & 45.05 & \textbf{27.96} & 37.94\\
% & \cellcolor{gray!30} Ours & \cellcolor{gray!30} 35.06 & \cellcolor{gray!30} \textbf{20.90} & \cellcolor{gray!30} 35.06 & \cellcolor{gray!30} 21.07 & \cellcolor{gray!30} 51.92 & \cellcolor{gray!30} \textbf{27.43} & \cellcolor{gray!30} 51.92 & \cellcolor{gray!30} 41.83 & \cellcolor{gray!30} 42.49 & \cellcolor{gray!30} 27.81 & \cellcolor{gray!30} \textbf{34.55} \\
\midrule

\multirow{4}{*}{CodeGen-2B} 
& Ori & 31.27 & 11.04 & 31.27 & 9.75 & 44.82 & 1.63 & 44.82 & 24.45 & 38.05 & 11.72 & 69.20 \\
& $\lossclm$ & 32.99 & 15.78 & 32.99 & 16.41 & 46.22 & 2.43 & 46.22 & 32.00 & \textbf{39.61} & 16.66 & 57.94 \\
& $\lossdataaug$ & 31.62 & 17.62 & 31.62 & 16.61 & 45.96 & $^{*}$\textbf{22.86} & 45.96 & \textbf{34.50} & 38.79 & 22.90 & 40.96 \\
& \cellcolor{gray!30} Ours & \cellcolor{gray!30} 31.56 & \cellcolor{gray!30} \textbf{$^{**}$19.21} & \cellcolor{gray!30} 31.56 & \cellcolor{gray!30} \textbf{17.12} & \cellcolor{gray!30} 45.04 & \cellcolor{gray!30} 21.92 & \cellcolor{gray!30} 45.04 & \cellcolor{gray!30} 34.36 & \cellcolor{gray!30} 38.30 & \cellcolor{gray!30} \textbf{23.15} & \cellcolor{gray!30} \textbf{39.56} \\
\midrule

\multirow{4}{*}{CodeGen-350M} 
& Ori & 17.10 & 3.57 & 17.10 & 3.06 & 26.75 & 1.11 & 26.75 & 9.54 & 21.93 & 4.32 & 80.30\\
& $\lossclm$ & 18.10 & 6.19 & 18.10 & 6.47 & 29.24 & 1.46 & 29.24 & 15.96 & 23.67 & 7.52 & 68.23 \\
& $\lossdataaug$ & 18.10 & 7.45 & 18.10 & 7.94 & 30.11 & 8.59 & 30.11 & 18.58 & 24.10 & 10.64 & 55.85 \\
% $\lossdataaug$ & 18.28 & 7.93 & 18.28 & 7.41 & 30.56 & 9.35 & 30.56 & 19.12 & 24.42 & 10.95 & 44.84 \\
& \cellcolor{gray!30} Ours & 
\cellcolor{gray!30} 18.33 & 
\cellcolor{gray!30} \textbf{$^{**}$9.72} & \cellcolor{gray!30} 18.33 & \cellcolor{gray!30} \textbf{8.05} & \cellcolor{gray!30} 31.04 & \cellcolor{gray!30} \textbf{$^{**}$10.67} & \cellcolor{gray!30} 31.04 & \cellcolor{gray!30} \textbf{$^{**}$21.58} & \cellcolor{gray!30} \textbf{24.69} & \cellcolor{gray!30} \textbf{12.51} & \cellcolor{gray!30} \textbf{49.33}\\

 
\bottomrule
\end{tabular}
}
\vspace{-1em}
    \label{tab:main_results}
\end{table*}


==> tables/motivation.tex <==
% \usepackage{tabularray}
\begin{table}
% \setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.}
\centering
    \caption{The ReCode~\citep{recode} robustness evaluation for SOTA public code models. \npsk shows the nominal pass@1 without perturbation; \rpskf shows the robust pass@1 under perturbation. The significant drop of Drop\% indicates unsatisfied robustness performance of these models.}
    \vspace{-0.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrr}
\toprule
\multicolumn{2}{c}{Transformation}  &  StarCoder & WizardCoder & CodeGen16B \\

\midrule
\multirow{3}{*}{Docstring} & \npsk & 
41.27 & 53.29 & 39.23 \\ 
& \rpskf & 11.60
& 20.43 & 15.81 \\
& \rdrop & 71.89 & 61.66 & 69.70 \\
\hline

\multirow{3}{*}{Function} & \npsk & 
41.27 & 53.29 & 39.23 \\ 
& \rpskf & 15.30 & 29.06 & 26.95 \\
& \rperct & 62.93 & 45.47 & 31.30 \\
\hline

\multirow{3}{*}{Syntax} & \npsk & 59.34 & 61.09 & 56.78 \\ 
& \rpskf & 4.21 & 9.86 & 5.54 \\
& \rperct & 92.91 & 83.86 & 90.24 \\
\hline

\multirow{3}{*}{Format} & \npsk & 59.34 & 61.09 & 56.78 \\ 
& \rpskf & 23.61 & 28.13 & 39.59 \\
& \rperct & 60.21 & 53.95 & 30.27 \\
% \hline

\bottomrule
\end{tabular}
}
\vspace{-1em}
    \label{tab:motivation}
\end{table}


==> tables/motivation_small.tex <==
% \usepackage{tabularray}
\begin{table}
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.}
\centering
\caption{We evaluate the robustness of SOTA public code models on ReCode~\citep{recode} benchmark. Under four types of semantic-preserving program transformations on the same MBPP evaluation set, we see significant drops of pass@1 rate over unperturbed ones. The results indicate unsatisfied robustness performance of SOTA models.}
% \myshang{This table and its caption are not very clear to me. what's the baseline that the drop in this table is comparing against? (todo: codegen16B)}\linbo{Maybe adding one column: clean accuracy?}
\vspace{-0.5em}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
Models & Docstring & Function & Syntax & Format\\
\midrule
StarCoder-15B & 71.89\%$\downarrow$ & 62.93\%$\downarrow$ & 92.91\%$\downarrow$ & 60.21\%$\downarrow$ \\
WizardCoder-15B & 61.66\%$\downarrow$ & 45.47\%$\downarrow$ & 83.86\%$\downarrow$ & 53.95\%$\downarrow$ \\
% CodeLlama-7B & 78.70\%$\downarrow$ & 69.37\%$\downarrow$ & 94.43\%$\downarrow$ & 62.36\%$\downarrow$\\

\bottomrule
\end{tabular}
}
    \vspace{-1em}
    \label{tab:motivation_small}
\end{table}

